Validated forward integration scheme for parabolic PDEs via Chebyshev series

In this paper we introduce a new approach to compute rigorously solutions of Cauchy problems for a class of semi-linear parabolic partial differential equations. Expanding solutions with Chebyshev series in time and Fourier series in space, we introduce a zero finding problem $F(a)=0$ on a Banach algebra $X$ of Fourier-Chebyshev sequences, whose solution solves the Cauchy problem. The challenge lies in the fact that the linear part $\mathcal{L} = DF(0)$ has an infinite block diagonal structure with blocks becoming less and less diagonal dominant at infinity. We introduce analytic estimates to show that $\mathcal{L}$ is an invertible linear operator on $X$, and we obtain explicit, rigorous and computable bounds for the operator norm $\| \mathcal{L}^{-1}\|_{B(X)}$. These bounds are then used to verify the hypotheses of a Newton-Kantorovich type argument which shows that the (Newton-like) operator $\mathcal{T}(a)=a - \mathcal{L}^{-1} F(a)$ is a contraction on a small ball centered at a numerical approximation of the Cauchy problem. The contraction mapping theorem yields a fixed point which corresponds to a classical (strong) solution of the Cauchy problem. The approach is simple to implement, numerically stable and is applicable to a class of PDE models, which include for instance Fisher's equation and the Swift-Hohenberg equation. We apply our approach to each of these models.

==> includes/cauchy_old.tex <==
We show that for a given $\varepsilon > 0$ and $\mu_k\geq 1$ there exists $N(\mu_k,\varepsilon)>2\mu_k$ (denote simply $N=N(\mu_k,\varepsilon)$), such that for any $N_1,N_2>N$ it holds that  
\[
\left\|\left(P_{N_1}\cL_kP_{N_1}\right)^{-1}-\left(P_{N_2}\cL_kP_{N_2}\right)^{-1}\right\|_{B(\ell^1)} < \varepsilon,
\]
here we think of $P_{N_1}\cL_kP_{N_1}$ and $P_{N_2}\cL_kP_{N_2}$ as infinite dimensional operators, the finite dimensional part padded with zeros.

Let $N_2>N_1$ (if $N_2=N_1$, then the difference is zero). Using \eqref{eqlkinvl3} we explicitly compute the difference $D=\left[\left(P_{N_1}\cL_kP_{N_1}\right)^{-1}-\left(P_{N_2}\cL_kP_{N_2}\right)^{-1}\right]$. For $i,l\leq N_1+1$ we have
\begin{multline*}
D_{i,l}=m_{i,l}-2\frac{ m_{i,1}\sum_{j=2}^{N_1+1}{(-1)^{j+1}m_{j,l}}}{1+2\sum_{j=2}^{N_1+1}{(-1)^{j+1}m_{j,1}}} - \left( \hat{m}_{i,l}-2\frac{ \hat{m}_{i,1}\sum_{j=2}^{N_2+1}{(-1)^{j+1}\hat{m}_{j,l}}}{1+2\sum_{j=2}^{N_2+1}{(-1)^{j+1}\hat{m}_{j,1}}}\right)=\\
%
%
%
\frac{2m_{i,1}\left(-2\sum_{j=2}^{N_1+1}{(-1)^{j+1}m_{j,l}}\sum_{j=N_1+2}^{N_2+1}{|\hat{m}_{j,1}|} + \sum_{j=N_1+2}^{N_2+1}{(-1)^{j+1}\hat{m}_{j,l}(1+2\sum_{j=2}^{N_1+1}{|m_{j,1}|})} \right)}{(1+2\sum_{j=2}^{N_1+1}{|m_{j,1}|})(1+2\sum_{j=2}^{N_2+1}{|\hat{m}_{j,1}|})}\leq\\
%
%
%
\frac{2|m_{i,1}|\left(2\sum_{j=2}^{N_1+1}{|m_{j,l}|}\sum_{j=N_1+2}^{N_2+1}{|\hat{m}_{j,1}|} + \sum_{j=N_1+2}^{N_2+1}{|\hat{m}_{j,l}|(1+2\sum_{j=2}^{N_1+1}{|m_{j,1}|})} \right)}{(1+2\sum_{j=2}^{N_1+1}{|m_{j,1}|})(1+2\sum_{j=2}^{N_2+1}{|\hat{m}_{j,1}|})},
\end{multline*}
where we used \eqref{eqpossum} and observation $m_{i,l}=\hat{m}_{j,1}$ for $i,l\leq N_1+1$ as $\left(P_{N_1}T_kP_{N_1}\right)^{-1}$ is independent on $P_{N_2}T_kP_{N_2}$.

Summing up $i=1,\dots,N_1$ we obtain
\begin{multline}
\label{eq:D1norm}
\|D_{\ro{1:N_1+1},\co{l}}\|_{B(\ell^1)} \leq 
\frac{(1+2\sum_{j=2}^{N_1+1}|m_{j,1}|)\left(2\sum_{j=2}^{N_1+1}{|m_{j,l}|}\sum_{j=N_1+2}^{N_2+1}{|\hat{m}_{j,1}|} + \sum_{j=N_1+2}^{N_2+1}{|\hat{m}_{j,l}|(1+2\sum_{j=2}^{N_1+1}{|m_{j,1}|})} \right)}{(1+2\sum_{j=2}^{N_1+1}{|m_{j,1}|})(1+2\sum_{j=2}^{N_2+1}{|\hat{m}_{j,1}|})}\leq\\
%
%
%
\sum_{j=2}^{N_1+1}{|m_{j,l}|}\frac{2\sum_{j=N_1+2}^{N_2+1}{|\hat{m}_{j,1}|}}{1+2\sum_{j=2}^{N_2+1}{|\hat{m}_{j,1}|}} + \sum_{j=N_1+2}^{N_2+1}{|\hat{m}_{j,l}|}=
%
%
%
\sum_{j=1}^{N_1}{|(T_k^{-1})_{j,l-1}|}\frac{2\sum_{j=N_1+1}^{N_2}{|\mu_k||(\hat{T}_k^{-1})_{j,1}|}}{1+2\sum_{j=1}^{N_2}{|\mu_k||(\hat{T}_k^{-1})_{j,1}|}} + \sum_{j=N_1+1}^{N_2}{|(\hat{T}_k^{-1})_{j,l-1}|}.
\end{multline}
It follows from Theorem~\ref{thm:trivialTkinvbd} that $\sum_{j=2}^{N}{|(T_k^{-1})_{j,l-1}|}$ is bounded by a constant (denote $C$) uniformly for all $N> 2\lfloor\mu_k\rfloor$. \eqref{eq:a1lower}.
\[
\|D_{\ro{1:N_1+1},\co{l}}\|_{B(\ell^1)} \leq 2C|\mu_k|\sum_{j=N_1+1}^{N_2}{|(\hat{T}_k^{-1})_{j,1}|} + \sum_{j=N_1+1}^{N_2}{|(\hat{T}_k^{-1})_{j,l-1}|} 
\]
as $N_1,N_2>2^p\mu_k$
from Lemma~\ref{lema2} it follows that 
\begin{equation}
\label{eq:cbd}
\sum_{j=N_1+1}^{N_2}{|(\hat{T}_k^{-1})_{j,1}|}, \sum_{j=N_1+1}^{N_2}{|(\hat{T}_k^{-1})_{j,l-1}|} < \left(\frac{1}{2^{p+1}}+\frac{1}{2^{2p+2}+1}\right)C.
\end{equation}
We estimate the remaining terms for $i=N_1+2,\dots,N_2$
\begin{multline*}
\|D_{\ro{N_1+2:N_2+1},\co{l}}\|_{1} \leq \sum_{i=N_1+2}^{N_2+1}|m_{i,l}|+2\frac{ \sum_{i=N_1+2}^{N_2+1}|m_{i,1}|\sum_{j=2}^{N_2+1}{|m_{j,l}|}}{1+2\sum_{j=2}^{N_2+1}{|m_{j,1}|}}=\\
%
%
%
\sum_{i=N_1+1}^{N_2}|(\hat{T}_k^{-1})_{i,l-1}|+2\frac{ \sum_{j=N_1+1}^{N_2}|\mu_k||(\hat{T}_k^{-1})_{j,1}|\sum_{j=1}^{N_2}{|(\hat{T}_k^{-1})_{j,l-1}|}}{1+2\sum_{j=1}^{N_2}{|\mu_k||(\hat{T}_k^{-1})_{j,1}|}} \leq \sum_{i=N_1+1}^{N_2}|(\hat{T}_k^{-1})_{i,l-1}| + 2C|\mu_k|\sum_{j=N_1+1}^{N_2}{|(\hat{T}_k^{-1})_{j,1}|}.
\end{multline*}
In overall using \eqref{eq:cbd} we have
\[
\|D_{\ro{1:N_2+1},\co{l}}\|_{B(\ell^1)} \leq 
4C^2|\mu_k|\left(\frac{1}{2^{p+1}}+\frac{1}{2^{2p+2}+1}\right) + 2C\left(\frac{1}{2^{p+1}}+\frac{1}{2^{2p+2}+1}\right)
\]
clearly there exists sufficiently large $p$, such that for $N>2^p\mu_k$ it holds that for $l\leq N_1+1$
\[
\|D_{\ro{1:N_2+1},\co{l}}\|_{B(\ell^1)} < \varepsilon.
\]

Whereas for $l>N_1+1$ we proceed using the overestimate \eqref{eq:lkinv_form}
\[
\|D_{\ro{1:N_2+1},\co{l}}\|_{B(\ell^1)} \leq 2\sum_{i=1}^{N_2}{|(T_k^{-1})_{i,l-1}|} \leq 2\left\|\widetilde{I}_{\co{c}}\right\|_{\ellmat} + 
2\mu_k|\widetilde{I}_{2c}|\left(\sum_{\substack{j=1\\j\neq n}}^{N/2}{a_j + \hat{a}_j}\right),
\]
where $n$ is such that $N_2-2n+c = l$, $\widetilde{I}$ is the corresponding diagonal block, we used \eqref{eq:totalbd}. As $l>N_1+1$, then by Lemma~\ref{lema2} all terms in $\widetilde{I}$ are bounded by $\frac{1}{2^{p+1}\mu_k}$, compare \eqref{eq:eqIbds} $\left|\widetilde{I}_{11}\right|< a_{n}, \left|\widetilde{I}_{12}\right|, \left|\widetilde{I}_{21}\right|<\hat{a}_{n},\left|\widetilde{I}_{22}\right|<b_{(N-2n+2)/2}$, hence pulling out $\frac{1}{2^{p+1}}$ 
\[
\|D_{\ro{1:N_2+1},\co{l}}\|_{B(\ell^1)} \leq \frac{1}{2^{p+1}}\widetilde{C}.
\]

Finally there exists sufficiently large $p$, such that for $N>2^p\mu_k$ it holds that
\[
\|\left(P_{N_1}\cL_kP_{N_1}\right)^{-1}-\left(P_{N_2}\cL_kP_{N_2}\right)^{-1}\|_{B(\ell^1)} < \varepsilon.
\]
